Drive Anywhere: Generalizable End-to-end Autonomous Driving with Multi-modal Foundation Models

As autonomous driving technology matures, end-to-end methodologies have emerged as a leading strategy, promising seamless integration from perception to control via deep learning. However, existing systems grapple with challenges such as unexpected open set environments and the complexity of black-box models. At the same time, the evolution of deep learning introduces larger, multimodal foundational models, offering multi-modal visual and textual understanding. In this paper, we harness these multimodal foundation models to enhance the robustness and adaptability of autonomous driving systems, enabling out-of-distribution, end-to-end, multimodal, and more explainable autonomy. Specifically, we present an approach to apply end-to-end open-set (any environment/scene) autonomous driving that is capable of providing driving decisions from representations queryable by image and text. To do so, we introduce a method to extract nuanced spatial (pixel/patch-aligned) features from transformers to enable the encapsulation of both spatial and semantic features. Our approach (i) demonstrates unparalleled results in diverse tests while achieving significantly greater robustness in out-of-distribution situations, and (ii) allows the incorporation of latent space simulation (via text) for improved training (data augmentation via text) and policy debugging. We encourage the reader to check our explainer video at https://www.youtube.com/watch?v=4n-DJf8vXxo&feature=youtu.be and to view the code and demos on our project webpage at https://drive-anywhere.github.io/.

==> sandbox/doodle.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{@{}c|ccccc|cccc@{}}
\toprule
\multirow{2}{*}{\textbf{Setting}} & \multicolumn{5}{c}{\textbf{Scenario}} & \multicolumn{4}{c}{\textbf{Methods}} \\
& Scene & Season & Weather & Time & Actor & CNN & CLIP & DINO & BLIP \\
\midrule
ID & Rural & Summer & Dry & Day & Cars & & & & \\
\midrule
\multirow{7}{*}{OOD} & \multirow{3}{*}{Rural} & Spring & \multirow{3}{*}{Dry} & Day & & & & & \\
&  & Summer &  & Night & & & & & \\
& & Fall &  & Day & & & & & \\
&  & Winter & Snow & Day & & & & & \\
& \multirow{3}{*}{Urban} & \multirow{3}{*}{Summer} & Dry & Day & & & & & \\
&  &  & Rain & Day & & & & & \\
&  &  & Dry & Night & & & & & \\
\bottomrule
\end{tabular}
\caption{\textbf{Out-of-distribution generalization.} \todo{description}.}
\label{tab:ood_generalization}
\end{table*}


\begin{table*}[ht]
\begin{minipage}{0.28\linewidth}
    \centering
    \includegraphics[width=\textwidth]{example-image-a}
\end{minipage}
\hfill
\begin{minipage}{0.7\linewidth}
    \centering
    \begin{tabular}{@{}c|ccccc|cccc@{}}
    \toprule
    \multirow{2}{*}{\textbf{Setting}} & \multicolumn{5}{c}{\textbf{Scenarios}} & \multicolumn{4}{c}{\textbf{Methods}} \\
    & Scene & Season & Weather & Time & Actor & CNN & CLIP & DINO & BLIP \\
    \midrule
    ID & Rural & Summer & Dry & Day & Car & & & & \\
    \midrule
    \multirow{14}{*}{OOD} & \multirow{6}{*}{Rural} & Spring & Dry & Day & Car$^\dagger$ & & & & \\
    &  & Summer & Dry & Night & Car$^\dagger$ & & & & \\
    & & Fall & Dry & Day & Car$^\dagger$ & & & & \\
    &  & Winter & Snow & Day & Car$^\dagger$ & & & & \\
    & & Spring & Dry & Day & Animal & & & & \\
    &  & Summer & Dry & Night & Animal & & & & \\
    & & Fall & Dry & Day & Animal & & & & \\
    &  & Winter & Snow & Day & Animal & & & & \\
    \cmidrule{2-6}
    & \multirow{6}{*}{Urban} & Summer & Dry & Day & Car$^\dagger$ & & & & \\
    &  & Summer & Rain & Day & Car$^\dagger$ & & & & \\
    &  & Summer & Dry & Night & Car$^\dagger$ & & & & \\
    &  & Summer & Dry & Day & Animal & & & & \\
    &  & Summer & Rain & Day & Animal & & & & \\
    &  & Summer & Dry & Night & Animal & & & & \\
    \bottomrule
    \end{tabular}
\end{minipage}
\caption{\textbf{Out-of-distribution generalization.} The left figures are illustrations for the scenarios. $^\dagger$indicates different car types. \textit{ID} is in distribution (evaluated on data not in the training dataset yet of the same scenario). \textit{OOD} is out-of-distribution.}
\label{tab:ood_generalization}
\end{table*}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.6\linewidth]{example-image-a}
    \caption{\textbf{Cross modality generalization.} \todo{A line plot with vertical axis as performance and horizontal axis as the ratio of cross-modality features used.}}
    \label{fig:cross_modality_generalization}
\end{figure}

\begin{table}[t]
    \centering
    \scriptsize
    \begin{tabular}{c||c|c|c}
        \toprule
        Image & Car, Road, Tree, Sky & + Car \& Road + Dark & + Car Parts \\
        \midrule
        0.99 & 0.27 & 0.54 & 0.66 \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{A debugging tool}. We use LLMs to propose potentially relevant concepts for language-augmented latent space simulation to inspect the decision making of a policy.}
    \label{tab:debugging_tool}
\end{table}


\begin{table}[t]
    \centering
    \scriptsize
    \begin{tabular}{l||c|c c c c c}
        \toprule
         \multirow{2}{*}{\textbf{Crashes}} & \multirow{2}{*}{\makecell{\textbf{Lane}\\ \textbf{Stable} }} & \multicolumn{5}{c}{\textbf{Obstacle Avoidance}} \\
         & & Pedestrian & Roadblock & Cone & Chair & House \\
        \hline
        No FM & 7.3 /km & 8/10 & 9/10 & 10/10 & 9/10 & 10/10 \\
        With FM & 0 /km & 0/10 & 0/10 & 0/10 & 0/10 & 1/10 \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Real Car Test}. \todo{description}.}
    \label{tab:real_car}
\end{table}

\subsection{Concept Prior from Global Context}

\begin{itemize}
    \item Use a set of pre-defined concepts (in the form of textual feature) to guide decision making.
    \item (Idea) Combine image-to-text-feature replacement with dropout to get uncertainty in control.
    \item (Idea) Somewhat amplify the feature that matches the pre-set concept; however, simply adding relevant feature to "activated" pixels does not seem right.
    \item (Idea) Do some evidence accumulation; not sure if it makes more sense to simply add temporal reasoning in the policy network.
\end{itemize}

